Reducing Drift in Structure From Motion Using Extended Features

Low-frequency long-range errors (drift) are an endemic problem in 3D structure from motion, and can often hamper reasonable reconstructions of the scene. In this paper, we present a method to dramatically reduce scale and positional drift by using extended structural features such as planes and vanishing points. Unlike traditional feature matches, our extended features are able to span non-overlapping input images, and hence provide long-range constraints on the scale and shape of the reconstruction. We add these features as additional constraints to a state-of-the-art global structure from motion algorithm and demonstrate that the added constraints enable the reconstruction of particularly drift-prone sequences such as long, low field-of-view videos without inertial measurements. Additionally, we provide an analysis of the drift-reducing capabilities of these constraints by evaluating on a synthetic dataset. Our structural features are able to significantly reduce drift for scenes that contain long-spanning man-made structures, such as aligned rows of windows or planar building facades.

==> figures/quantitative.tex <==
\begin{figure}
\begin{subfigure}{\linewidth}
  \hfill\includegraphics[width=\linewidth]{figures/images/rotation_error.pdf}
  \caption{Rotational drift: We see that the added constraints practically remove the observed rotational drift, and without the added constraints, even bundle adjustment has difficulty converging on the correct solution.}
  \label{fig:rotation_error}
\end{subfigure}% <-- added
\medskip

\begin{subfigure}{\linewidth}
  \hfill\includegraphics[width=0.982\linewidth]{figures/images/position_error.pdf}
  \caption{Positional drift: We see that bundle adjustment universally decreases error across all reconstructions, but cannot fully correct for the positional drift even after the rotational drift has been removed. One unit along the vertical axis is equal to the baseline between a pair of cameras.}
  \label{fig:position_error}
\end{subfigure}
\label{fig:synthetic_error}
\caption{{\bf Quantitative evaluation}: A comparison of rotational (a) and positional (b) drift using different combinations of Theia with global bundle adjustment (BA), our vanishing point constraints (VP), and our planar constraints (Plane). In order to be robust to pose errors in individual frames, we align the reconstructions to ground truth by estimating a similarity transformation between the first 200 camera centers. As a result, the lowest error (best aligned orientation) is not necessarily at the first frame. }
\end{figure}
